See Less, Specify More: Visual Evidence Budgets for Generalizable VLAs

Generalization remains a central bottleneck for vision-language-action (VLA) models: under distractors, appearance shifts, and semantically similar tasks, the policy must often infer local execution details from coarse instructions while also deciding which parts of the image matter for control. We present S2 (See Less, Specify More), a framework for improving VLA generalization by training the executor under a cleaner interface. Specify More preserves the original instruction as a stable high-level goal while relabeling each trajectory into refined trajectory- and subtask-level language that disambiguates the current execution mode. Unlike native attention, See Less imposes an explicit visual evidence budget, training the executor to act from task-sufficient evidence rather than unconstrained visual context, without any region or mask annotation. This interface lets the executor follow detailed guidance without relying on distracting visual patches or resolving avoidable ambiguity on its own, and it remains compatible with off-the-shelf VLM planners through in-context learning. Across our main evaluation settings, S2 improves overall generalization metrics by changing the executor's learning problem: coarse instructions induce avoidable supervision aliasing, goal-preserving local guidance outperforms instruction replacement in our main ablations, and explicit evidence budgeting reduces dependence on broad visual context beyond efficiency considerations. Across eight real-robot tasks on TX-G2 (an AgiBot G2-compatible variant) and HSR, S2 raises mean subtask success from 54.2% to 79.0% over pi0.5. Together, these results suggest that VLA generalization improves when the executor is trained to act from informative local guidance and task-sufficient visual evidence, rather than recovering both from weak supervision.

==> sections/00_abstract.tex <==
\begin{abstract}
Generalization remains a central bottleneck for vision-language-action (VLA)
models: under distractors, appearance shifts, and semantically similar tasks,
the policy must often infer local execution details from coarse instructions
while also deciding which parts of the image matter for control. We present
\stwoname{} (\seelessname{}, \specifymorename{}), a framework for improving VLA
generalization by training the executor under a cleaner interface.
\specifymorename{} preserves the original instruction as a stable high-level
goal while relabeling each trajectory into refined trajectory- and
subtask-level language that disambiguates the current execution mode.
Unlike native attention, \seelessname{} imposes an explicit visual evidence
budget, training the executor to act from task-sufficient evidence rather than
unconstrained visual context, without any region or mask annotation. This
interface lets the executor follow detailed guidance without relying on
distracting visual patches or resolving avoidable ambiguity on its own, and it
remains compatible with off-the-shelf VLM planners through in-context learning.
Across our main evaluation settings, S2 improves overall generalization
metrics by changing the
executor's learning problem: coarse instructions induce avoidable supervision
aliasing, goal-preserving local guidance outperforms instruction
replacement in our main ablations, and explicit evidence budgeting reduces
dependence on broad visual
context beyond efficiency considerations. Across eight real-robot tasks on
TX-G2 (an AgiBot G2-compatible variant) and HSR, S2 raises mean
subtask success from 54.2\% to 79.0\% over $\pi_{0.5}$. Together, these
results suggest that VLA
generalization improves when the executor is trained to act from informative
local guidance and task-sufficient visual evidence, rather than recovering
both from weak supervision.
\end{abstract}


==> sections/05_limitations.tex <==
\section{Limitations}
The full S2 pipeline currently assumes offline relabeling and subtask
alignment for the language-side supervision. More broadly, \stwoname{} is
intended to reduce specification-induced ambiguity and nuisance dependence,
not to resolve all sources of multimodality in robot control.

